NGTS-EB-7, an eccentric, long-period, low-mass eclipsing binary

Despite being the most common types of stars in the Galaxy, the physical properties of late M dwarfs are often poorly constrained. A trend of radius inflation compared to evolutionary models has been observed for earlier type M dwarfs in eclipsing binaries, possibly caused by magnetic activity. It is currently unclear whether this trend also extends to later type M dwarfs below the convective boundary. This makes the discovery of lower-mass, fully convective, M dwarfs in eclipsing binaries valuable for testing evolutionary models especially in longer-period binaries where tidal interaction between the primary and secondary is negligible. With this context, we present the discovery of the NGTS-EB-7 AB system, an eclipsing binary containing a late M dwarf secondary and an evolved G-type primary star. The secondary star has a radius of $0.125 \pm 0.006 R_\odot$ , a mass of $0.096 \pm 0.004 M_\odot$ and follows a highly eccentric $(e=0.71436 \pm 0.00085)$ orbit every $193.35875 \pm 0.00034$ days. This makes NGTS-EB-7 AB the third longest-period eclipsing binary system with a secondary smaller than $200 M_J$ with the mass and radius constrained to better than $5 \%$. In addition, NGTS-EB-7 is situated near the centre of the proposed LOPS2 southern field of the upcoming PLATO mission, allowing for detection of the secondary eclipse and measurement of the companion`s temperature. With its long-period and well-constrained physical properties - NGTS-EB-7 B will make a valuable addition to the sample of M dwarfs in eclipsing binaries and help in determining accurate empirical mass/radius relations for later M dwarf stars.

==> Tables/t_circs_table.tex <==
\begin{tabular}{c c c}
	\toprule
	$\log_{10}{Q_\text{A}}$ & $\log_{10}{Q_\text{B}}$ & $\tau_e$ (Gyr)\\
	\hline
	4.5&4.5&$2.21\times10^{4}$\\
	4.5&5.0&$2.21\times10^{4}$\\
	4.5&5.5&$2.21\times10^{4}$\\
	4.5&6.0&$2.21\times10^{4}$\\
	5.0&4.5&$6.97\times10^{4}$\\
	5.0&5.0&$6.99\times10^{4}$\\
	5.0&5.5&$6.99\times10^{4}$\\
	5.0&6.0&$7.0\times10^{4}$\\
	5.5&4.5&$2.19\times10^{5}$\\
	5.5&5.0&$2.21\times10^{5}$\\
	5.5&5.5&$2.21\times10^{5}$\\
	5.5&6.0&$2.21\times10^{5}$\\
	6.0&4.5&$6.78\times10^{5}$\\
	6.0&5.0&$6.93\times10^{5}$\\
	6.0&5.5&$6.97\times10^{5}$\\
	6.0&6.0&$6.99\times10^{5}$\\
	7.0&4.5&$5.31\times10^{6}$\\
	7.0&5.0&$6.36\times10^{6}$\\
	7.0&5.5&$6.78\times10^{6}$\\
	7.0&6.0&$6.93\times10^{6}$\\
	\bottomrule
\end{tabular}
